Learning Universal Predictors

Meta-learning has emerged as a powerful approach to train neural networks to learn new tasks quickly from limited data. Broad exposure to different tasks leads to versatile representations enabling general problem solving. But, what are the limits of meta-learning? In this work, we explore the potential of amortizing the most powerful universal predictor, namely Solomonoff Induction (SI), into neural networks via leveraging meta-learning to its limits. We use Universal Turing Machines (UTMs) to generate training data used to expose networks to a broad range of patterns. We provide theoretical analysis of the UTM data generation processes and meta-training protocols. We conduct comprehensive experiments with neural architectures (e.g. LSTMs, Transformers) and algorithmic data generators of varying complexity and universality. Our results suggest that UTM data is a valuable resource for meta-learning, and that it can be used to train neural networks capable of learning universal prediction strategies.

==> context-table-unfiltered.tex <==
\begin{tabular}{l|l|l|l|l|l|l|l|l}
ctx          & \bfcode{<}               & \bfcode{>}               & \bfcode{+}               & \bfcode{-}               & \bfcode{[}               & \bfcode{]}               & \bfcode{\{}              & \bfcode{.}               \\
\hline
\bfcode{}    & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!65}.25  \\
\bfcode{+}   & \cellcolor{blue!54}.21  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!39}.15  & \cellcolor{blue!3}.01   & \cellcolor{blue!0}.01   & \cellcolor{blue!67}.26  \\
\bfcode{-}   & \cellcolor{blue!49}.19  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!52}.2   & \cellcolor{blue!36}.14  & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!70}.27  \\
\bfcode{.}   & \cellcolor{blue!49}.19  & \cellcolor{blue!49}.19  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!59}.23  \\
\bfcode{<}   & \cellcolor{blue!62}.24  & \cellcolor{blue!3}.01   & \cellcolor{blue!62}.24  & \cellcolor{blue!54}.21  & \cellcolor{blue!3}.01   & \cellcolor{blue!0}.01    & \cellcolor{blue!0}.01   & \cellcolor{blue!75}.29  \\
\bfcode{>}   & \cellcolor{blue!3}.01   & \cellcolor{blue!54}.21  & \cellcolor{blue!62}.24  & \cellcolor{blue!59}.23  & \cellcolor{blue!0}.01    & \cellcolor{blue!0}.01    & \cellcolor{blue!0}.01   & \cellcolor{blue!80}.31  \\
\bfcode{++}  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!36}.14  & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!65}.25  \\
\bfcode{+.}  & \cellcolor{blue!39}.15  & \cellcolor{blue!42}.16  & \cellcolor{blue!39}.15  & \cellcolor{blue!39}.15  & \cellcolor{blue!29}.11  & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!54}.21  \\
\bfcode{+<}  & \cellcolor{blue!52}.2   & \cellcolor{blue!3}.01   & \cellcolor{blue!52}.2   & \cellcolor{blue!49}.19  & \cellcolor{blue!13}.05  & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!72}.28  \\
\bfcode{+>}  & \cellcolor{blue!3}.01   & \cellcolor{blue!49}.19  & \cellcolor{blue!52}.2   & \cellcolor{blue!49}.19  & \cellcolor{blue!13}.05  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!72}.28  \\
\bfcode{+[}  & \cellcolor{blue!44}.17  & \cellcolor{blue!39}.15  & \cellcolor{blue!42}.16  & \cellcolor{blue!47}.18  & \cellcolor{blue!26}.1   & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!57}.22  \\
\bfcode{+]}  & \cellcolor{blue!42}.16  & \cellcolor{blue!42}.16  & \cellcolor{blue!42}.16  & \cellcolor{blue!42}.16  & \cellcolor{blue!3}.01   & \cellcolor{blue!21}.08  & \cellcolor{blue!3}.01  & \cellcolor{blue!67}.26  \\
\bfcode{+\{} & \cellcolor{blue!39}.15  & \cellcolor{blue!62}.24  & \cellcolor{blue!52}.2   & \cellcolor{blue!36}.14  & \cellcolor{blue!3}.01   & \cellcolor{blue!26}.1   & \cellcolor{blue!3}.01  & \cellcolor{blue!39}.15  \\
\bfcode{--}  & \cellcolor{blue!44}.17  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!49}.19  & \cellcolor{blue!31}.12  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!65}.25  \\
\bfcode{-.}  & \cellcolor{blue!39}.15  & \cellcolor{blue!42}.16  & \cellcolor{blue!39}.15  & \cellcolor{blue!39}.15  & \cellcolor{blue!29}.11  & \cellcolor{blue!18}.07  & \cellcolor{blue!0}.01   & \cellcolor{blue!54}.21  \\
\bfcode{-<}  & \cellcolor{blue!49}.19  & \cellcolor{blue!3}.01   & \cellcolor{blue!49}.19  & \cellcolor{blue!52}.2   & \cellcolor{blue!13}.05  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!72}.28  \\
\bfcode{->}  & \cellcolor{blue!3}.01   & \cellcolor{blue!52}.2   & \cellcolor{blue!52}.2   & \cellcolor{blue!49}.19  & \cellcolor{blue!11}.04  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!72}.28  \\
\bfcode{-[}  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!24}.09  & \cellcolor{blue!0}.01    & \cellcolor{blue!0}.01   & \cellcolor{blue!59}.23  \\
\bfcode{-]}  & \cellcolor{blue!47}.18  & \cellcolor{blue!44}.17  & \cellcolor{blue!39}.15  & \cellcolor{blue!44}.17  & \cellcolor{blue!6}.02   & \cellcolor{blue!21}.08  & \cellcolor{blue!3}.01  & \cellcolor{blue!57}.22  \\
\bfcode{-\{} & \cellcolor{blue!42}.16  & \cellcolor{blue!52}.2   & \cellcolor{blue!42}.16  & \cellcolor{blue!59}.23  & \cellcolor{blue!3}.01   & \cellcolor{blue!18}.07  & \cellcolor{blue!0}.01   & \cellcolor{blue!44}.17  \\
\bfcode{.+}  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!49}.19  & \cellcolor{blue!3}.01   & \cellcolor{blue!29}.11  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!65}.25  \\
\bfcode{.-}  & \cellcolor{blue!47}.18  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!47}.18  & \cellcolor{blue!31}.12  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!67}.26  \\
\bfcode{..}  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!13}.05  & \cellcolor{blue!13}.05  & \cellcolor{blue!0}.01   & \cellcolor{blue!57}.22  \\
\bfcode{.<}  & \cellcolor{blue!49}.19  & \cellcolor{blue!3}.01   & \cellcolor{blue!52}.2   & \cellcolor{blue!52}.2   & \cellcolor{blue!13}.05  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!70}.27  \\
\bfcode{.>}  & \cellcolor{blue!3}.01   & \cellcolor{blue!52}.2   & \cellcolor{blue!49}.19  & \cellcolor{blue!52}.2   & \cellcolor{blue!13}.05  & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!72}.28  \\
\bfcode{.[}  & \cellcolor{blue!47}.18  & \cellcolor{blue!39}.15  & \cellcolor{blue!44}.17  & \cellcolor{blue!47}.18  & \cellcolor{blue!21}.08  & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!57}.22  \\
\bfcode{.]}  & \cellcolor{blue!42}.16  & \cellcolor{blue!47}.18  & \cellcolor{blue!42}.16  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!24}.09  & \cellcolor{blue!3}.01  & \cellcolor{blue!57}.22  \\
\bfcode{.\{} & \cellcolor{blue!42}.16  & \cellcolor{blue!44}.17  & \cellcolor{blue!70}.27  & \cellcolor{blue!57}.22  & \cellcolor{blue!3}.01   & \cellcolor{blue!6}.02   & \cellcolor{blue!3}.01  & \cellcolor{blue!36}.14  \\
\bfcode{<+}  & \cellcolor{blue!49}.19  & \cellcolor{blue!49}.19  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!34}.13  & \cellcolor{blue!13}.05  & \cellcolor{blue!3}.01  & \cellcolor{blue!65}.25  \\
\bfcode{<-}  & \cellcolor{blue!49}.19  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!47}.18  & \cellcolor{blue!31}.12  & \cellcolor{blue!13}.05  & \cellcolor{blue!3}.01  & \cellcolor{blue!67}.26  \\
\bfcode{<.}  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!8}.03   & \cellcolor{blue!18}.07  & \cellcolor{blue!0}.01   & \cellcolor{blue!57}.22  \\
\bfcode{<<}  & \cellcolor{blue!52}.2   & \cellcolor{blue!3}.01   & \cellcolor{blue!52}.2   & \cellcolor{blue!52}.2   & \cellcolor{blue!8}.03   & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!75}.29  \\
\bfcode{<[}  & \cellcolor{blue!49}.19  & \cellcolor{blue!42}.16  & \cellcolor{blue!44}.17  & \cellcolor{blue!47}.18  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!54}.21  \\
\bfcode{<]}  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!39}.15  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!24}.09  & \cellcolor{blue!3}.01  & \cellcolor{blue!59}.23  \\
\bfcode{<\{} & \cellcolor{blue!57}.22  & \cellcolor{blue!24}.09  & \cellcolor{blue!47}.18  & \cellcolor{blue!57}.22  & \cellcolor{blue!3}.01   & \cellcolor{blue!21}.08  & \cellcolor{blue!3}.01  & \cellcolor{blue!49}.19  \\
\bfcode{>+}  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!31}.12  & \cellcolor{blue!13}.05  & \cellcolor{blue!3}.01  & \cellcolor{blue!70}.27  \\
\bfcode{>-}  & \cellcolor{blue!47}.18  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!47}.18  & \cellcolor{blue!31}.12  & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!70}.27  \\
\bfcode{>.}  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!8}.03   & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!57}.22  \\
\bfcode{>>}  & \cellcolor{blue!3}.01   & \cellcolor{blue!54}.21  & \cellcolor{blue!54}.21  & \cellcolor{blue!49}.19  & \cellcolor{blue!8}.03   & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!70}.27  \\
\bfcode{>[}  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!24}.09  & \cellcolor{blue!0}.01    & \cellcolor{blue!0}.01   & \cellcolor{blue!59}.23  \\
\bfcode{>]}  & \cellcolor{blue!44}.17  & \cellcolor{blue!42}.16  & \cellcolor{blue!42}.16  & \cellcolor{blue!42}.16  & \cellcolor{blue!3}.01   & \cellcolor{blue!24}.09  & \cellcolor{blue!3}.01  & \cellcolor{blue!62}.24  \\
\bfcode{>\{} & \cellcolor{blue!26}.1   & \cellcolor{blue!39}.15  & \cellcolor{blue!54}.21  & \cellcolor{blue!62}.24  & \cellcolor{blue!3}.01   & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!54}.21  \\
\bfcode{[+}  & \cellcolor{blue!39}.15  & \cellcolor{blue!42}.16  & \cellcolor{blue!42}.16  & \cellcolor{blue!3}.01   & \cellcolor{blue!13}.05  & \cellcolor{blue!67}.26  & \cellcolor{blue!3}.01  & \cellcolor{blue!52}.2   \\
\bfcode{[-}  & \cellcolor{blue!39}.15  & \cellcolor{blue!39}.15  & \cellcolor{blue!3}.01   & \cellcolor{blue!39}.15  & \cellcolor{blue!16}.06  & \cellcolor{blue!65}.25  & \cellcolor{blue!8}.03  & \cellcolor{blue!52}.2   \\
\bfcode{[.}  & \cellcolor{blue!36}.14  & \cellcolor{blue!36}.14  & \cellcolor{blue!36}.14  & \cellcolor{blue!36}.14  & \cellcolor{blue!18}.07  & \cellcolor{blue!59}.23  & \cellcolor{blue!0}.01   & \cellcolor{blue!36}.14  \\
\bfcode{[<}  & \cellcolor{blue!44}.17  & \cellcolor{blue!3}.01   & \cellcolor{blue!34}.13  & \cellcolor{blue!34}.13  & \cellcolor{blue!8}.03   & \cellcolor{blue!75}.29  & \cellcolor{blue!6}.02  & \cellcolor{blue!57}.22  \\
\bfcode{[>}  & \cellcolor{blue!3}.01   & \cellcolor{blue!42}.16  & \cellcolor{blue!36}.14  & \cellcolor{blue!36}.14  & \cellcolor{blue!8}.03   & \cellcolor{blue!72}.28  & \cellcolor{blue!6}.02  & \cellcolor{blue!57}.22  \\
\bfcode{[[}  & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!47}.18  & \cellcolor{blue!49}.19  & \cellcolor{blue!21}.08  & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!49}.19  \\
\bfcode{]+}  & \cellcolor{blue!49}.19  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!34}.13  & \cellcolor{blue!16}.06  & \cellcolor{blue!3}.01  & \cellcolor{blue!62}.24  \\
\bfcode{]-}  & \cellcolor{blue!44}.17  & \cellcolor{blue!52}.2   & \cellcolor{blue!3}.01   & \cellcolor{blue!47}.18  & \cellcolor{blue!31}.12  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!62}.24  \\
\bfcode{].}  & \cellcolor{blue!39}.15  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!47}.18  & \cellcolor{blue!3}.01   & \cellcolor{blue!21}.08  & \cellcolor{blue!0}.01   & \cellcolor{blue!57}.22  \\
\bfcode{]<}  & \cellcolor{blue!57}.22  & \cellcolor{blue!3}.01   & \cellcolor{blue!44}.17  & \cellcolor{blue!44}.17  & \cellcolor{blue!13}.05  & \cellcolor{blue!24}.09  & \cellcolor{blue!3}.01  & \cellcolor{blue!72}.28  \\
\bfcode{]>}  & \cellcolor{blue!3}.01   & \cellcolor{blue!49}.19  & \cellcolor{blue!54}.21  & \cellcolor{blue!49}.19  & \cellcolor{blue!16}.06  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01  & \cellcolor{blue!67}.26  \\
\bfcode{][}  & \cellcolor{blue!34}.13  & \cellcolor{blue!49}.19  & \cellcolor{blue!54}.21  & \cellcolor{blue!72}.28  & \cellcolor{blue!6}.02   & \cellcolor{blue!3}.01   & \cellcolor{blue!3}.01  & \cellcolor{blue!39}.15  \\
\bfcode{]]}  & \cellcolor{blue!42}.16  & \cellcolor{blue!52}.2   & \cellcolor{blue!44}.17  & \cellcolor{blue!42}.16  & \cellcolor{blue!3}.01   & \cellcolor{blue!21}.08  & \cellcolor{blue!3}.01  & \cellcolor{blue!54}.21  \\
\bfcode{\{+} & \cellcolor{blue!57}.22  & \cellcolor{blue!39}.15  & \cellcolor{blue!18}.07  & \cellcolor{blue!3}.01   & \cellcolor{blue!16}.06  & \cellcolor{blue!80}.31  & \cellcolor{blue!3}.01  & \cellcolor{blue!44}.17  \\
\bfcode{\{-} & \cellcolor{blue!39}.15  & \cellcolor{blue!36}.14  & \cellcolor{blue!3}.01   & \cellcolor{blue!34}.13  & \cellcolor{blue!8}.03   & \cellcolor{blue!72}.28  & \cellcolor{blue!3}.01  & \cellcolor{blue!65}.25  \\
\bfcode{\{.} & \cellcolor{blue!52}.2   & \cellcolor{blue!24}.09  & \cellcolor{blue!34}.13  & \cellcolor{blue!65}.25  & \cellcolor{blue!3}.01   & \cellcolor{blue!21}.08  & \cellcolor{blue!3}.01  & \cellcolor{blue!59}.23  \\
\bfcode{\{<} & \cellcolor{blue!29}.11  & \cellcolor{blue!3}.01   & \cellcolor{blue!47}.18  & \cellcolor{blue!52}.2   & \cellcolor{blue!18}.07  & \cellcolor{blue!57}.22  & \cellcolor{blue!6}.02  & \cellcolor{blue!49}.19  \\
\bfcode{\{>} & \cellcolor{blue!3}.01   & \cellcolor{blue!42}.16  & \cellcolor{blue!59}.23  & \cellcolor{blue!36}.14  & \cellcolor{blue!11}.04  & \cellcolor{blue!44}.17  & \cellcolor{blue!6}.02  & \cellcolor{blue!59}.23  \\
\bfcode{\{]} & \cellcolor{blue!24}.09  & \cellcolor{blue!8}.03   & \cellcolor{blue!57}.22  & \cellcolor{blue!75}.29  & \cellcolor{blue!3}.01   & \cellcolor{blue!8}.03   & \cellcolor{blue!3}.01  & \cellcolor{blue!83}.32  \\
avg          & \cellcolor{green!39}.15 & \cellcolor{green!39}.15 & \cellcolor{green!39}.15 & \cellcolor{green!42}.16 & \cellcolor{green!16}.06 & \cellcolor{green!24}.09 & \cellcolor{green!3}.01 & \cellcolor{green!59}.23 \\
\end{tabular}

==> context-table.tex <==
\begin{tabular}{|c|lllllll|l|} 
\hline
Context                  & \multicolumn{1}{c|}{\bfcode{<}} & \multicolumn{1}{c|}{\bfcode{>}} & \multicolumn{1}{c|}{\bfcode{+}} & \multicolumn{1}{c|}{\bfcode{-}} & \multicolumn{1}{c|}{\bfcode{[}} & \multicolumn{1}{c|}{\bfcode{]}} & \multicolumn{1}{c|}{\bfcode{.}} & Freq.                   \\
\cline{1-2}\bfcode{\_\_} & \cellcolor{blue!49}.19          & \cellcolor{blue!49}.19          & \cellcolor{blue!49}.19          & \cellcolor{blue!52}.20          & \cellcolor{blue!0}.00           & \cellcolor{blue!0}.00           & \cellcolor{blue!59}.23          & \cellcolor{red!28}.018  \\
\cline{1-2}\bfcode{\_+}  & \cellcolor{blue!57}.22          & \cellcolor{blue!62}.24          & \cellcolor{blue!49}.19          & \cellcolor{blue!0}.00           & \cellcolor{blue!29}.11          & \cellcolor{blue!0}.00           & \cellcolor{blue!62}.24          & \cellcolor{red!7}.004   \\
\cline{1-2}\bfcode{\_-}  & \cellcolor{blue!39}.15          & \cellcolor{blue!70}.27          & \cellcolor{blue!0}.00           & \cellcolor{blue!54}.21          & \cellcolor{blue!34}.13          & \cellcolor{blue!0}.00           & \cellcolor{blue!62}.24          & \cellcolor{red!7}.004   \\
\cline{1-2}\bfcode{\_.}  & \cellcolor{blue!44}.17          & \cellcolor{blue!57}.22          & \cellcolor{blue!54}.21          & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!0}.00           & \cellcolor{blue!59}.23          & \cellcolor{red!7}.004   \\
\cline{1-2}\bfcode{\_<}  & \cellcolor{blue!59}.23          & \cellcolor{blue!0}.00           & \cellcolor{blue!72}.28          & \cellcolor{blue!59}.23          & \cellcolor{blue!0}.00           & \cellcolor{blue!0}.00           & \cellcolor{blue!67}.26          & \cellcolor{red!7}.004   \\
\cline{1-2}\bfcode{\_>}  & \cellcolor{blue!0}.00           & \cellcolor{blue!47}.18          & \cellcolor{blue!44}.17          & \cellcolor{blue!67}.26          & \cellcolor{blue!0}.00           & \cellcolor{blue!0}.00           & \cellcolor{blue!100}.39         & \cellcolor{red!5}.003   \\
\cline{1-2}\bfcode{++}   & \cellcolor{blue!49}.19          & \cellcolor{blue!44}.17          & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!39}.15          & \cellcolor{blue!16}.06          & \cellcolor{blue!67}.26          & \cellcolor{red!35}.023  \\
\cline{1-2}\bfcode{+.}   & \cellcolor{blue!39}.15          & \cellcolor{blue!34}.13          & \cellcolor{blue!36}.14          & \cellcolor{blue!34}.13          & \cellcolor{blue!29}.11          & \cellcolor{blue!21}.08          & \cellcolor{blue!67}.26          & \cellcolor{red!60}.039  \\
\cline{1-2}\bfcode{+<}   & \cellcolor{blue!47}.18          & \cellcolor{blue!0}.00           & \cellcolor{blue!49}.19          & \cellcolor{blue!49}.19          & \cellcolor{blue!13}.05          & \cellcolor{blue!24}.09          & \cellcolor{blue!77}.30          & \cellcolor{red!38}.025  \\
\cline{1-2}\bfcode{+>}   & \cellcolor{blue!0}.00           & \cellcolor{blue!49}.19          & \cellcolor{blue!49}.19          & \cellcolor{blue!47}.18          & \cellcolor{blue!16}.06          & \cellcolor{blue!24}.09          & \cellcolor{blue!75}.29          & \cellcolor{red!37}.024  \\
\cline{1-2}\bfcode{+[}   & \cellcolor{blue!42}.16          & \cellcolor{blue!36}.14          & \cellcolor{blue!39}.15          & \cellcolor{blue!36}.14          & \cellcolor{blue!31}.12          & \cellcolor{blue!3}.01           & \cellcolor{blue!72}.28          & \cellcolor{red!31}.020  \\
\cline{1-2}\bfcode{+]}   & \cellcolor{blue!31}.12          & \cellcolor{blue!44}.17          & \cellcolor{blue!44}.17          & \cellcolor{blue!42}.16          & \cellcolor{blue!6}.02           & \cellcolor{blue!29}.11          & \cellcolor{blue!65}.25          & \cellcolor{red!10}.006  \\
\cline{1-2}\bfcode{--}   & \cellcolor{blue!44}.17          & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!44}.17          & \cellcolor{blue!39}.15          & \cellcolor{blue!18}.07          & \cellcolor{blue!70}.27          & \cellcolor{red!37}.024  \\
\cline{1-2}\bfcode{-.}   & \cellcolor{blue!36}.14          & \cellcolor{blue!39}.15          & \cellcolor{blue!34}.13          & \cellcolor{blue!36}.14          & \cellcolor{blue!29}.11          & \cellcolor{blue!24}.09          & \cellcolor{blue!62}.24          & \cellcolor{red!61}.040  \\
\cline{1-2}\bfcode{-<}   & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!52}.20          & \cellcolor{blue!49}.19          & \cellcolor{blue!18}.07          & \cellcolor{blue!21}.08          & \cellcolor{blue!75}.29          & \cellcolor{red!38}.025  \\
\cline{1-2}\bfcode{->}   & \cellcolor{blue!0}.00           & \cellcolor{blue!52}.20          & \cellcolor{blue!47}.18          & \cellcolor{blue!52}.20          & \cellcolor{blue!13}.05          & \cellcolor{blue!21}.08          & \cellcolor{blue!75}.29          & \cellcolor{red!37}.024  \\
\cline{1-2}\bfcode{-[}   & \cellcolor{blue!42}.16          & \cellcolor{blue!36}.14          & \cellcolor{blue!36}.14          & \cellcolor{blue!39}.15          & \cellcolor{blue!34}.13          & \cellcolor{blue!3}.01           & \cellcolor{blue!70}.27          & \cellcolor{red!29}.019  \\
\cline{1-2}\bfcode{-]}   & \cellcolor{blue!47}.18          & \cellcolor{blue!47}.18          & \cellcolor{blue!47}.18          & \cellcolor{blue!49}.19          & \cellcolor{blue!3}.01           & \cellcolor{blue!16}.06          & \cellcolor{blue!52}.20          & \cellcolor{red!11}.007  \\
\cline{1-2}\bfcode{.+}   & \cellcolor{blue!44}.17          & \cellcolor{blue!42}.16          & \cellcolor{blue!42}.16          & \cellcolor{blue!0}.00           & \cellcolor{blue!31}.12          & \cellcolor{blue!24}.09          & \cellcolor{blue!77}.30          & \cellcolor{red!63}.041  \\
\cline{1-2}\bfcode{.-}   & \cellcolor{blue!44}.17          & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!44}.17          & \cellcolor{blue!29}.11          & \cellcolor{blue!24}.09          & \cellcolor{blue!75}.29          & \cellcolor{red!61}.040  \\
\cline{1-2}\bfcode{..}   & \cellcolor{blue!36}.14          & \cellcolor{blue!39}.15          & \cellcolor{blue!42}.16          & \cellcolor{blue!39}.15          & \cellcolor{blue!16}.06          & \cellcolor{blue!29}.11          & \cellcolor{blue!59}.23          & \cellcolor{red!100}.066 \\
\cline{1-2}\bfcode{.<}   & \cellcolor{blue!47}.18          & \cellcolor{blue!0}.00           & \cellcolor{blue!49}.19          & \cellcolor{blue!44}.17          & \cellcolor{blue!13}.05          & \cellcolor{blue!26}.10          & \cellcolor{blue!80}.31          & \cellcolor{red!60}.039  \\
\cline{1-2}\bfcode{.>}   & \cellcolor{blue!0}.00           & \cellcolor{blue!42}.16          & \cellcolor{blue!47}.18          & \cellcolor{blue!47}.18          & \cellcolor{blue!13}.05          & \cellcolor{blue!31}.12          & \cellcolor{blue!80}.31          & \cellcolor{red!63}.041  \\
\cline{1-2}\bfcode{.[}   & \cellcolor{blue!36}.14          & \cellcolor{blue!39}.15          & \cellcolor{blue!36}.14          & \cellcolor{blue!44}.17          & \cellcolor{blue!29}.11          & \cellcolor{blue!3}.01           & \cellcolor{blue!72}.28          & \cellcolor{red!29}.019  \\
\cline{1-2}\bfcode{.]}   & \cellcolor{blue!42}.16          & \cellcolor{blue!44}.17          & \cellcolor{blue!42}.16          & \cellcolor{blue!42}.16          & \cellcolor{blue!3}.01           & \cellcolor{blue!21}.08          & \cellcolor{blue!67}.26          & \cellcolor{red!29}.019  \\
\cline{1-2}\bfcode{<+}   & \cellcolor{blue!49}.19          & \cellcolor{blue!47}.18          & \cellcolor{blue!42}.16          & \cellcolor{blue!0}.00           & \cellcolor{blue!42}.16          & \cellcolor{blue!11}.04          & \cellcolor{blue!70}.27          & \cellcolor{red!40}.026  \\
\cline{1-2}\bfcode{<-}   & \cellcolor{blue!54}.21          & \cellcolor{blue!42}.16          & \cellcolor{blue!0}.00           & \cellcolor{blue!47}.18          & \cellcolor{blue!34}.13          & \cellcolor{blue!16}.06          & \cellcolor{blue!67}.26          & \cellcolor{red!38}.025  \\
\cline{1-2}\bfcode{<.}   & \cellcolor{blue!36}.14          & \cellcolor{blue!42}.16          & \cellcolor{blue!36}.14          & \cellcolor{blue!39}.15          & \cellcolor{blue!8}.03           & \cellcolor{blue!29}.11          & \cellcolor{blue!70}.27          & \cellcolor{red!64}.042  \\
\cline{1-2}\bfcode{<<}   & \cellcolor{blue!47}.18          & \cellcolor{blue!0}.00           & \cellcolor{blue!49}.19          & \cellcolor{blue!49}.19          & \cellcolor{blue!13}.05          & \cellcolor{blue!24}.09          & \cellcolor{blue!77}.30          & \cellcolor{red!37}.024  \\
\cline{1-2}\bfcode{<[}   & \cellcolor{blue!36}.14          & \cellcolor{blue!42}.16          & \cellcolor{blue!44}.17          & \cellcolor{blue!42}.16          & \cellcolor{blue!29}.11          & \cellcolor{blue!3}.01           & \cellcolor{blue!65}.25          & \cellcolor{red!13}.008  \\
\cline{1-2}\bfcode{<]}   & \cellcolor{blue!36}.14          & \cellcolor{blue!44}.17          & \cellcolor{blue!42}.16          & \cellcolor{blue!47}.18          & \cellcolor{blue!3}.01           & \cellcolor{blue!29}.11          & \cellcolor{blue!59}.23          & \cellcolor{red!19}.012  \\
\cline{1-2}\bfcode{>+}   & \cellcolor{blue!47}.18          & \cellcolor{blue!42}.16          & \cellcolor{blue!49}.19          & \cellcolor{blue!0}.00           & \cellcolor{blue!36}.14          & \cellcolor{blue!16}.06          & \cellcolor{blue!70}.27          & \cellcolor{red!38}.025  \\
\cline{1-2}\bfcode{>-}   & \cellcolor{blue!44}.17          & \cellcolor{blue!47}.18          & \cellcolor{blue!0}.00           & \cellcolor{blue!44}.17          & \cellcolor{blue!39}.15          & \cellcolor{blue!13}.05          & \cellcolor{blue!72}.28          & \cellcolor{red!41}.027  \\
\cline{1-2}\bfcode{>.}   & \cellcolor{blue!36}.14          & \cellcolor{blue!36}.14          & \cellcolor{blue!42}.16          & \cellcolor{blue!42}.16          & \cellcolor{blue!13}.05          & \cellcolor{blue!26}.10          & \cellcolor{blue!65}.25          & \cellcolor{red!64}.042  \\
\cline{1-2}\bfcode{>>}   & \cellcolor{blue!0}.00           & \cellcolor{blue!47}.18          & \cellcolor{blue!47}.18          & \cellcolor{blue!54}.21          & \cellcolor{blue!13}.05          & \cellcolor{blue!24}.09          & \cellcolor{blue!75}.29          & \cellcolor{red!38}.025  \\
\cline{1-2}\bfcode{>[}   & \cellcolor{blue!39}.15          & \cellcolor{blue!39}.15          & \cellcolor{blue!39}.15          & \cellcolor{blue!44}.17          & \cellcolor{blue!29}.11          & \cellcolor{blue!3}.01           & \cellcolor{blue!67}.26          & \cellcolor{red!11}.007  \\
\cline{1-2}\bfcode{>]}   & \cellcolor{blue!42}.16          & \cellcolor{blue!39}.15          & \cellcolor{blue!39}.15          & \cellcolor{blue!47}.18          & \cellcolor{blue!3}.01           & \cellcolor{blue!24}.09          & \cellcolor{blue!67}.26          & \cellcolor{red!20}.013  \\
\cline{1-2}\bfcode{[+}   & \cellcolor{blue!44}.17          & \cellcolor{blue!36}.14          & \cellcolor{blue!36}.14          & \cellcolor{blue!0}.00           & \cellcolor{blue!31}.12          & \cellcolor{blue!34}.13          & \cellcolor{blue!77}.30          & \cellcolor{red!19}.012  \\
\cline{1-2}\bfcode{[-}   & \cellcolor{blue!44}.17          & \cellcolor{blue!29}.11          & \cellcolor{blue!0}.00           & \cellcolor{blue!42}.16          & \cellcolor{blue!24}.09          & \cellcolor{blue!39}.15          & \cellcolor{blue!83}.32          & \cellcolor{red!20}.013  \\
\cline{1-2}\bfcode{[.}   & \cellcolor{blue!39}.15          & \cellcolor{blue!44}.17          & \cellcolor{blue!42}.16          & \cellcolor{blue!36}.14          & \cellcolor{blue!26}.10          & \cellcolor{blue!3}.01           & \cellcolor{blue!70}.27          & \cellcolor{red!35}.023  \\
\cline{1-2}\bfcode{[<}   & \cellcolor{blue!39}.15          & \cellcolor{blue!0}.00           & \cellcolor{blue!31}.12          & \cellcolor{blue!34}.13          & \cellcolor{blue!18}.07          & \cellcolor{blue!54}.21          & \cellcolor{blue!83}.32          & \cellcolor{red!19}.012  \\
\cline{1-2}\bfcode{[>}   & \cellcolor{blue!0}.00           & \cellcolor{blue!39}.15          & \cellcolor{blue!26}.10          & \cellcolor{blue!36}.14          & \cellcolor{blue!18}.07          & \cellcolor{blue!54}.21          & \cellcolor{blue!85}.33          & \cellcolor{red!19}.012  \\
\cline{1-2}\bfcode{[[}   & \cellcolor{blue!36}.14          & \cellcolor{blue!34}.13          & \cellcolor{blue!44}.17          & \cellcolor{blue!36}.14          & \cellcolor{blue!24}.09          & \cellcolor{blue!0}.00           & \cellcolor{blue!85}.33          & \cellcolor{red!16}.010  \\
\cline{1-2}\bfcode{[]}   & \cellcolor{blue!29}.11          & \cellcolor{blue!29}.11          & \cellcolor{blue!85}.33          & \cellcolor{blue!29}.11          & \cellcolor{blue!0}.00           & \cellcolor{blue!16}.06          & \cellcolor{blue!72}.28          & \cellcolor{red!2}.001   \\
\cline{1-2}\bfcode{]+}   & \cellcolor{blue!42}.16          & \cellcolor{blue!39}.15          & \cellcolor{blue!42}.16          & \cellcolor{blue!0}.00           & \cellcolor{blue!36}.14          & \cellcolor{blue!39}.15          & \cellcolor{blue!62}.24          & \cellcolor{red!16}.010  \\
\cline{1-2}\bfcode{]-}   & \cellcolor{blue!34}.13          & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!39}.15          & \cellcolor{blue!39}.15          & \cellcolor{blue!44}.17          & \cellcolor{blue!59}.23          & \cellcolor{red!17}.011  \\
\cline{1-2}\bfcode{].}   & \cellcolor{blue!39}.15          & \cellcolor{blue!49}.19          & \cellcolor{blue!42}.16          & \cellcolor{blue!49}.19          & \cellcolor{blue!3}.01           & \cellcolor{blue!21}.08          & \cellcolor{blue!57}.22          & \cellcolor{red!25}.016  \\
\cline{1-2}\bfcode{]<}   & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!44}.17          & \cellcolor{blue!42}.16          & \cellcolor{blue!18}.07          & \cellcolor{blue!36}.14          & \cellcolor{blue!75}.29          & \cellcolor{red!14}.009  \\
\cline{1-2}\bfcode{]>}   & \cellcolor{blue!0}.00           & \cellcolor{blue!49}.19          & \cellcolor{blue!49}.19          & \cellcolor{blue!49}.19          & \cellcolor{blue!13}.05          & \cellcolor{blue!31}.12          & \cellcolor{blue!67}.26          & \cellcolor{red!17}.011  \\
\cline{1-2}\bfcode{][}   & \cellcolor{blue!34}.13          & \cellcolor{blue!34}.13          & \cellcolor{blue!26}.10          & \cellcolor{blue!70}.27          & \cellcolor{blue!26}.10          & \cellcolor{blue!0}.00           & \cellcolor{blue!70}.27          & \cellcolor{red!2}.001   \\
\cline{1-2}\bfcode{]]}   & \cellcolor{blue!34}.13          & \cellcolor{blue!52}.20          & \cellcolor{blue!44}.17          & \cellcolor{blue!44}.17          & \cellcolor{blue!0}.00           & \cellcolor{blue!24}.09          & \cellcolor{blue!62}.24          & \cellcolor{red!8}.005   \\
\hline Freq.             & \cellcolor{green!52}.14         & \cellcolor{green!52}.14         & \cellcolor{green!52}.14         & \cellcolor{green!56}.15         & \cellcolor{green!30}.08         & \cellcolor{green!30}.08         & \cellcolor{green!100}.27        &                         \\
\hline
\end{tabular}

